Inferring Hierarchical Mixture Structures: A Bayesian Nonparametric Approach

This paper focuses on the problem of hierarchical non-overlapping clustering of a dataset. In such a clustering, each data item is associated with exactly one leaf node and each internal node is associated with all the data items stored in the sub-tree beneath it, so that each level of the hierarchy corresponds to a partition of the dataset. We develop a novel Bayesian nonparametric method combining the nested Chinese Restaurant Process (nCRP) and the Hierarchical Dirichlet Process (HDP). Compared with other existing Bayesian approaches, our solution tackles data with complex latent mixture features which has not been previously explored in the literature. We discuss the details of the model and the inference procedure. Furthermore, experiments on three datasets show that our method achieves solid empirical results in comparison with existing algorithms.

==> experiments_copy.tex <==
\section{Experimental Observations}
For qualitative analysis, we use the following datasets: \texttt{Compound}~\cite{ClusteringDatasets}, \texttt{Animals}~\cite{kemp2008discovery} and \texttt{MNIST-fashion}~\cite{xiao2017fmnist}.
%
%This section demonstrates  our method using the following datasets from which some qualitative analysis of the output of the method can be obtained: Compound\footnote{\url{http://cs.uef.fi/sipu/datasets/}}~\cite{ClusteringDatasets}, Animals~\cite{kemp2008discovery} and MNIST-Fashion~\cite{xiao2017fmnist}.
Following this, we carry out a quantitative analysis for the \texttt{Amazon} text data~\cite{He2016ups} since it contains the cluster labels of all the items at multiple levels.

In the following experiments, we fix $H$ to be the Normal-inverse-Wishart (NIW) distribution and unsurprisingly $F$ is set as Gaussian.
% Further, denoting the inverse Wishart with $\mathcal{W}^{-1}$, $\NIW(\nu, \lambda,  \mu_0, \Sigma_0)$ samples $\phi = (\mu, \Sigma)$ by $\mu \sim \N(\mu_0, \frac 1 {\lambda} \Sigma)$ and $\Sigma \sim \mathcal{W}^{-1}(\Sigma_0, \nu)$.
% Let $\mu_0$ and $\Sigma_0$ be fixed to the empirical mean and covariance of the data.
% We manually set $L$ for each distinct dataset.
For more complex cases, one can consider the theoretical results of the effective length of the nCRP (see Proposition 3.1 in~\cite{Steinhardt2012}).
Due to the space limit, we leave discussion of the hyperparameters for all datasets in the supplemental material.

%
% \subsection{Posterior Predictive Checking}
% For a Bayesian model, sampling from the posterior predictive distribution is a basic model check~\cite{gelman2013bayesian}.
% Before analysing the performance, we conduct this fundamental study to check if the generated data under the model look similar to the observations.
% % \begin{figure}[!ht]
% % \centering
% % \includegraphics[scale=.15]{figures/compound}
% % \caption{Compound dataset}
% % \label{fg:compound}
% % \end{figure}
% The procedure is to draw a number of random samples, after inferring the parameters of the model.
% In particular, we draw 399 (equal to the dataset size) samples from the model learned for the Compound dataset.
% In~\Cref{fg:post-checking}, there are three independent draws from the posterior. One can see that the qualitative structure of the original dataset is present in the resampled data.
% \begin{figure}[!ht]
% \centering
% \subfloat[\texttt{Compound}]{
%     \includegraphics[scale=.095]{figures/compound.pdf}
% }
% \quad
% \subfloat[Sample 1]{
%     \includegraphics[scale=.095]{figures/post_sample1.pdf}
% }
% \subfloat[Sampe 2]{
%     \includegraphics[scale=.095]{figures/post_sample2.pdf}
% }
% \quad
% \subfloat[Sample 3]{
%     \includegraphics[scale=.095]{figures/post_sample3.pdf}
% }
% \caption{Sampling from posterior distribution}
% \label{fg:post-checking}
% \end{figure}
%
% \subsection{Convergence Analysis}
% Here we examine the convergence of the algorithm using \texttt{Animals}.
% \Cref{fg:conv} shows the unnormalised log likelihood for three individual simulations.
% It is observable that they converge to a certain satisfactory level after just a few hundred runs (far less than 500).
% Although it still increases afterwards, the rate of increase becomes slower.
% \begin{figure}[ht]
% \centering
% \includegraphics[scale=.3]{figures/animal_conv}
% \caption{Convergence plots on the \texttt{Animals} dataset}
% \label{fg:conv}
% \end{figure}

\subsection{Results}
\paragraph{\texttt{Animals}}
This dataset contains 102 binary features, e.g. ``has 6 legs'', ``lives in water'', ``bad temper'', etc.
Observing the heat-map of the empirical covariance of the data, there are not many influential features.
Hence, we employ Principal Component Analysis (PCA)~\cite{murphy2012machine} to reduce it to a five-dimensional feature space.
The MCMC burns $5,000$ runs and then reports the one with the greatest complete data likelihood $p(X, \bm{c}, V \mid B, \bm{\phi}, \Theta)$ among the following $100$ draws~\cite{adams2010tree}.

\begin{figure}[ht]
\centering
\includegraphics[scale=1.9]{./figures/animals_candidate_mcl_10.eps}
\caption{The tree of \texttt{Animals}}
\label{fg:animal}
\end{figure}

In~\Cref{fg:animal}, at the first level, from left to right, we see that the first big cluster contains the bird family.
The third one contains non-insects and non-birds and is further split between the reptiles and the mammals.
They are grouped together because they have lungs and teeth and are predators; on the other hand, they share a lot of negative features: ``they have no feathers'', ``do not eat nuts'', and ``do not live in houses'', etc.
Finally, the fifth cluster contains the insects and the herbivore mammals.
Overall, the clusters separate reasonably, and the purity of the clusters is reasonably good.

\begin{figure*}
\centering
\includegraphics[scale=0.5]{./figures/mnist-fashion-mcl-5-inkscape}
% \subfloat[$\alpha=.5, \gamma_0=5, \gamma=.05, L=4, \lambda=.01, \nu=200$\label{fg:fmnist-a}]{
%   \includegraphics[scale=0.71]{./figures/mnist-fashion-mcl-5-inkscape.pdf}
% }
% \\
% \subfloat[$\alpha=.35, \gamma_0=5, \gamma=1.5, L=4, \lambda=.02, \nu=200$\label{fg:fmnist-b}]{
%   \includegraphics[scale=0.71]{./figures/mnist-fashion-mcl-4-inkscape.pdf}
% }
\caption{The tree of \texttt{MNIST-fashion}}
\label{fg:fmnist}
\end{figure*}

\paragraph{\texttt{MNIST-fashion}}
This data is a collection of fashion images.
Each image is represented as a $28 \times 28$ vector of grayscale pixel values.
For better visualisation, we sample 100 samples evenly from each class.
PCA transforms the data to 22 dimensions via the asymptotic root mean square optimal threshold~\cite{Gavish2014} for keeping the singular values.
Using the same criterion as for Animal, we output two hierarchies with two sets of hyperparameters.
We set $\alpha=0.5, \gamma_0=5, \gamma=0.05, L=4, \lambda=0.01, \nu=200$.
This executes $2,500$ burn-in runs.

% At first glance,~\Cref{fg:fmnist-a} illustrates a significant property of the CRP which is ``the rich get richer''.
% However,~\Cref{fg:fmnist-b} shows that it is also possible to have a more even grouping by changing the hyperparameters.
% As it is grayscale data, in addition to the shape of the items, other factors affecting the clustering might be, e.g., the foreground/background colour area, the percentage of non-black colours in the image, the darkness/lightness of the item, etc.
% The two hierarchies both exhibit rather reasonable structures.
% Some mislabeled items are expected in a clustering task.

\Cref{fg:fmnist} illustrates a significant property of the CRP which is ``the rich get richer''.
As it is grayscale data, in addition to the shape of the items, other factors affecting the clustering might be, e.g., the foreground/background colour area, the percentage of non-black colours in the image, the darkness/lightness of the item, etc.
The hierarchical structure forms a hierarchy with high purity per level.
Some mislabeled items are expected in a clustering task.

\paragraph{\texttt{Amazon}}
This data incorporates the information such as images, descriptions and reviews of  products in the Amazon catalogue.
We uniformly downsample the indices in the fashion category and reserve $2,303$ entries from the data, which contain textual information about items such as their titles and descriptions\footnote{\url{http://jmcauley.ucsd.edu/data/amazon}: the data is available upon request.}.
% However, the sampled identities for the data entries are providable}.
The data is preprocessed via the method in~\cite{Gavish2014}  and only $190$ features are kept, formed as the Term Frequency and Inverse Document Frequency (TF-IDF) of the items' titles and descriptions.

Our evaluation applies the methodology in~\cite{Kuang2013} to compare the clustering results against the ground-truth labels level by level.
We compare 6 levels, which is the maximum branch length of the items in the ground truth.
When extracting the labels from the trees (either for the algorithm outputs or the ground truth), items that are on a path of length less than 6 are extended to level 6 by assigning the same cluster label as that in their last level to the remaining levels up to 6.
This is to keep the consistency of the number of items for computing metrics at each level.

For the comparison, we first consider the gold standard AC with Ward distance~\cite{ward1963hierarchical}.
We adopt the existing implementations for PERCH and PYDT\footnote{\url{https://github.com/iesl/xcluster} and \url{https://github.com/davidaknowles/pydt}}.
For PYDT which is sensitive to the hyperparameters, we applied the authors' implemented hyperparameter optimisation to gather the hyperparameters prior to running the repeated simulations.
At each level, we consider four different evaluation metrics, namely, the purity, the normalised mutual information (NMI), the adjusted rand index (ARI), and the F-Measure~\cite{karypis2000comparison}.
Level 1 is the level for the root node.
Each algorithm was repeated 35 times.

\begin{figure}[!ht]
\centering
\includegraphics[scale=.32]{./figures/amazon_after_pca-results.pdf}
\caption{Metrics on \texttt{Amazon} by levels}\label{fg:amazon-results}
\end{figure}

\Cref{fg:amazon-results} is plotted with  $95\%$ confidence intervals, although the uncertainty is rather small.
It depicts that our method achieves clearly better scores with respect to purity and NMI.
In the figure, PYDT-SL and PYDT-MH correspond to the slice and the MH sampling solution, respectively.
As the tree approaches to a lower level, our method also achieves a better performance in F-measure.
For ARI, despite that PERCH performs the best, all numerical values are exceedingly close to $0$.
However, some theoretical work of~\cite{romano2016adjusting} suggests that ARI is more preferred in the scenario that the data contains big and equal-sized clusters.
This is opposed to our ground truth which is highly unbalanced among the clusters at each level.
BHMC does show the potential to perform well according to certain traditional metrics.


==> hyper.tex <==
\section{Hyperparameters}
% In both sampling schemes, we can further add a Metropolis-Hastings step to update the hyperparameters.
% That is, we take advantage of the posterior $\post$ for the original tree and $\post'$ for the newly generated tree.
% It follows that we can have the acceptance rate
% \begin{align*}
% A = \min \left[1, ~\frac {\post'} {\post} \frac {q(Z \pvert Z')} {q(Z' \pvert Z)} \right] \,.
% \end{align*}
% In the sequel, the acceptance rate serves as a threshold for randomly accepting the new tree.
% In general, $q(\cdot)$ is a proposal distribution and can also be symmetric and further be canceled.

Let use denote the gamma distribution by $\Ga(\cdot)$.
We specify the hyperparameters as follows
\begin{align*}
\alpha & \sim \Ga(2, 1) \quad \gamma_0 \sim \Ga(5, 1) \quad \gamma \sim \B(2, 1) \\
L & = \ceil{l} \quad s.t.\quad l \sim \Ga(3, 0.7) + 1 \, .
\end{align*}
The distribution for the maximum levels $L$ is chosen to entail that $3$ and $4$ would appear the most frequently---we assume the most hierarchies have only three to four necessary levels.
For more complex case, one can consider the theoretical results of the effective length (see in Proposition 3.1) of nCRP in \citep{Steinhardt2012}.
Even though, the practitioners are allowed to choose their priors according to their domain knowledge about the data.

We can view the base measure $H$ as the prior to the density function $f$.
Therefore we choose a common pair as
\begin{align*}
H & = \NIW(\mu_0, \lambda, \Phi, \nu) \\
f(x \pvert \phi) &= \N(x; \mu, \Sigma) \quad i.e.~ \phi = (\mu, \Sigma) \,.
\end{align*}
$\NIW$ is the Normal-Inverse-Wishart which is usually considered the prior for a normal distribution.
We could use the empirical mean and covariance matrix of the data for $\mu_0$ and $\Phi$ respectively.
In the procedure, a covariance $\Sigma'$ for a mixture is first drawn from the inverse Wishart with the scale $1/\nu$, which means the mixture's covariance will be numerically smaller if $\nu$ is large.
Later, the mixture mean is sampled from a Gaussian such that $\mu' \sim \N(\mu, \Sigma' / \lambda)$.
For a strategy for picking the scales, we would like to see the data can be grouped into $K$ components, and hence we set the scale $\nu$ for the mixture covariance larger than $K$.
Then, we also would like to see the mixture mean across all the possible region, and thus could set $\lambda$ to satisfy   $\lambda \nu \approx 1$.

In both sampling schemes, we can further add a Metropolis-Hastings step to update the hyperparameters.
That is, we take advantage of the posterior $\post$ for the original tree and $\post'$ for the newly generated tree.


==> relatedwork.tex <==
\section{Related Work}
We focus on Bayesian methods for the HC.
\cite{stolcke1993hidden} first applied marginal likelihood as the standard for merging the clusters with Agglomerative clustering (AC).
A Bayesian AC with the objective of maximising the \emph{posteriori} was investigated in~\cite{iwayama1995hierarchical}; however, the model assumptions of independence between the data and the clusters are strong.
% \cite{ramoni2002cluster} handled  time series data by maximising the marginal likelihood in an online fashion.
Furthermore, \cite{segal2002prob} presented a Bayesian algorithm assuming that each node associates with a model and similar models should be placed together.
% In another domain,~\cite{friedman2003pcluster} was proposed to doubly cluster the rows and columns in gene data and assign the data entries into a hierarchy.
A Bayesian hierarchical clustering (BHC) that integrates the statistical hypothesis into the traditional AC was proposed in ~\cite{heller2005bhc} and, more
recently, BHC has been relaxed into a non-probabilistic formulation via conjugate-exponential
models~\cite{lee2015bayesian}.
% Interestingly, to address the users' need, an alternative tool is to merge the user interactions into the BHC~\cite{vikram2016interactive}.
However, BHC only provides a Bayesian method of clustering the items into a hierarchy rather than a Bayesian model with a generative process for the data.

In light of hierarchical generative models, an early Bayesian solution introduced the Gaussian tree generative process~\cite{williams2000mcmc}, such that each non-root node is sampled from a Gaussian distribution with the mean of the parent node and predefined level-wise covariances.
The leaf nodes are the observations.
The number of nodes at a certain level is based on a Poisson distribution considering the number of nodes in the parent level.

{\color{red}
A number of works have proposed different but related ways to construct hierarchical tree priors. For example, \cite{Knowles2015} developed the Pitman-Yor Diffusion Tree (PYDT) which is a generalisation of the Dirichlet diffusion tree (DDT)~\cite{neal2003density}.
It assumes that all the observations go through a random walk process from time $0$ to $1$, and each observation has a probability of diverging from the path at the end of each interval of length $dt$ where $0 < dt < 1$.
Finally at time $1$, the data items are sampled from a Gaussian distribution.
With the divergence at different time points, a tree prior is then constructed such that earlier diverging points are the parent nodes of  later diverging points.
In PYDT, the diverging point is also distributed to a Gaussian with the mean of the previous diverging point of the path and some time-related variance.
\cite{teh2008bayesian} proposed applying the Kingman's coalescent as a prior to the HC.
It is in spirit similar to DDT and PYDT, however it is a backward generative process.

A very general way to construct a hierarchical tree prior is proposed in~\cite{adams2010tree} which proposes the tree-structured stick-breaking construction (TSSB) of a hierarchical tree of parameters,  a generalisation of the nested Chinese Restaurant Process (nCRP)~\cite{blei2010nested}.  The method we propose falls within the framework of the TSSB and we discuss in more detail in the next section.}

%They interleave two stick-breaking processes to generate a HC which may maintain observations at internal nodes. It is a very similar configuration to the PYDT, for obtaining parameters for one node from its parent node, although it assumes fixed variance through the path.
%Moreover, the nCRP is largely overlapped by the PYDT and the data can be sampled from internal nodes in the PYDT as well.

\cite{paisley2015nested} discussed the nested Hierarchical Dirichlet Process (nHDP) for topic modelling which, similar to the method we present here, uses the nCRP to navigate through the hierarchy, but associates nodes in the tree with topics. The nHDP first generates a global topic tree using the nCRP~\cite{blei2010nested} where each node relates to one atom (topic) drawn from the base distribution.
\cite{Ahmed2013} also proposed a model that is very similar to nHDP, but appealed to a different inference procedures.
% and applied it in a different scope of applications.

\subsection{Comparison to our Work}
TSSB focuses on Gaussian for the internal nodes in the tree; however, our internal nodes are mixture distributions.
A mixture distribution can handle the data better in many cases, as a single distribution like Gaussian can be considered as a mixture with a single component, and thus the mixture distribution provides more flexibility.
Our implemented model is most closely connected to the TSSB.
Despite its additional complexity, our model still achieves an elegant closed-form updates for the parameters while TSSB needs to apply Hamiltonian Monte Carlo to update the internal parameters in addition to their core slice sampler.

The proposed model exploits the nCRP and HDP and so, at first glance, can appear similar to the nHDP.  It is important to point out that the original nCRP and nHDP are models for hierarchical topic modelling.
Hierarchical topic modelling is well distinguished from HC in~\cite{blei2010nested}.
In HC, the internal nodes are summarisations of the children, while in a topic hierarchy, an internal node reflects the shared terminology of documents associated with the path to that node.  Most notably, a \emph{one-level} HDP is applied in nHDP for projecting a global topic tree to a local, document-specific, one. In contrast, we develop a hierarchy of mixture components and connect these components through a \emph{multilevel} HDP along each path in the hierarchy, thus employing the HDP for a very different purpose.


==> source code/abstract.tex <==
\begin{abstract}
% This paper focuses on the problem of hierarchical non-overlapping clustering of a dataset. In such a clustering, each data item is associated with exactly one leaf node and each internal node is associated with all the data items stored in the sub-tree beneath it, so that each level of the hierarchy corresponds to a partition of the dataset.
% We develop a novel Bayesian nonparametric method combining the nested Chinese Restaurant Process (nCRP) and the Hierarchical Dirichlet Process (HDP).     %., which we motivate through a ``Chinese Hierarchical Franchise Process'' (CHFP) metaphor.
% Compared with other existing Bayesian approaches, our solution tackles data with complex latent mixture features which has not been previously explored in the literature.
% We discuss the details of the model and the inference procedure.
% Furthermore, experiments on three real-world datasets show that our method achieves solid empirical results.


We present a Bayesian Nonparametric model for Hierarchical Clustering (HC).
Such a model has two main components.
The first component is the random walk process from parent to child in the hierarchy and we apply nested Chinese Restaurant Process (nCRP).
Then, the second part is the diffusion process from parent to child where we employ Hierarchical Dirichlet Process Mixture Model (HDPMM).
This is different from the common choice which is Gaussian-to-Gaussian.
We demonstrate the properties of the model and propose a Markov Chain Monte Carlo procedure with elegantly analytical updating steps for inferring the model variables.
Experiments on the real-world datasets show that our method obtains reasonable hierarchies and remarkable empirical results according to some well known metrics.
\end{abstract}


==> source code/conclusion.tex <==
\section{Conclusion}
This paper has discussed a new perspective for Bayesian nonparametric HC.
Our model, BHMC, develops an infinitely branching hierarchy of mixture parameters, that are linked along paths in the hierarchy through a multilevel HDP.
A nested CRP is used to select a path in the hierarchy and mixture components are drawn from the mixture distribution in the leaf node of the selected path.
The evaluation shows that BHMC is able to provide good hierarchical clustering results on three real-world datasets with different types of characteristics (i.e., binary, visual and textual) and clearly performs better than other methods with respect to purity and NMI on the Amazon dataset with ground truth, which shows the promising potential of the model.

% In future work, it will be interesting to explore the non-exchangeable Bayesian models in hopes of improving the approach.
% Additionally, we will seek solutions to handle big data applications based on BHMC.
%{\color{blue}
%In future work, we would like to enhance the model to  handle big data applications based on BHMC.
%}


==> source code/experiments.tex <==
\section{Experiments}
For qualitative analysis, we use the datasets: \texttt{Animals}~\cite{kemp2008discovery} and \texttt{MNIST-fashion}~\cite{xiao2017fmnist}.
Following this, we carry out a quantitative analysis for the \texttt{Amazon} text data~\cite{He2016ups} since it contains the cluster labels of all the items at multiple levels.
% \footnote{We leave further details of the experimental setup to the supplemental material.}.
% We apply Principal Component Analysis (PCA) to truncate \texttt{Animals} and \texttt{MNIST-fashion} to 7 dimensions and 10 dimensions respectively.
% This data incorporates the information such as images, descriptions and reviews of  products in the Amazon catalogue.
% We uniformly down-sample the indices in the fashion category and reserve $2,303$ entries from the data, which contain textual information about items such as their titles and descriptions\footnote{\url{http://jmcauley.ucsd.edu/data/amazon}: the data is available upon request.}.
% The data is preprocessed via the method in~\cite{Gavish2014}  and only $190$ features are kept, formed as the Term Frequency and Inverse Document Frequency (TF-IDF) of the items' titles and descriptions.

We fix the parameters for $H$ as
$\bm{\mu}_0 = \m{0}$ and $\m{\Sigma}_0 = \m{I}$.
Additionally, we set the covariance matrix for $F$ as $\m{\Sigma} = \sigma^2 \m{I}$.
We set the number of levels $L$ intuitively based on the data.
For more complex cases, one can consider the theoretical results of the effective length of the nCRP~\cite{Steinhardt2012}.

%
% \subsection{Posterior Predictive Checking}
% For a Bayesian model, sampling from the posterior predictive distribution is a basic model check~\cite{gelman2013bayesian}.
% Before analysing the performance, we conduct this fundamental study to check if the generated data under the model look similar to the observations.
% % \begin{figure}[!ht]
% % \centering
% % \includegraphics[scale=.15]{figures/compound}
% % \caption{Compound dataset}
% % \label{fg:compound}
% % \end{figure}
% The procedure is to draw a number of random samples, after inferring the parameters of the model.
% In particular, we draw 399 (equal to the dataset size) samples from the model learned for the Compound dataset.
% In~\Cref{fg:post-checking}, there are three independent draws from the posterior. One can see that the qualitative structure of the original dataset is present in the resampled data.
% \begin{figure}[!ht]
% \centering
% \subfloat[\texttt{Compound}]{
%     \includegraphics[scale=.095]{figures/compound.pdf}
% }
% \quad
% \subfloat[Sample 1]{
%     \includegraphics[scale=.095]{figures/post_sample1.pdf}
% }
% \subfloat[Sampe 2]{
%     \includegraphics[scale=.095]{figures/post_sample2.pdf}
% }
% \quad
% \subfloat[Sample 3]{
%     \includegraphics[scale=.095]{figures/post_sample3.pdf}
% }
% \caption{Sampling from posterior distribution}
% \label{fg:post-checking}
% \end{figure}

\subsection{Convergence Analysis}
We examine the convergence of the algorithm using \texttt{Animals}.
\Cref{fg:conv} shows the unnormalised log likelihood for five individual simulations.
The simulations quickly reach a certain satisfactory level.
Apart from that, the fluctuation shows that the algorithm keeps searching the solution space over the iterations.


\subsection{Results}
\paragraph{\texttt{Animals}}
This dataset contains 102 binary features, e.g. ``has 6 legs'', ``lives in water'', ``bad temper'', etc.
Observing the heat-map of the empirical covariance of the data, there are not many influential features.
Hence, we employ Principal Component Analysis (PCA)~\cite{murphy2012machine} to reduce it to a seven-dimensional feature space.
The MCMC burns $500$ runs and then reports the one with the greatest complete data likelihood $p(\data, \bm{c}, \m{V} \mid \m{B}, \bm{\theta})$ amongst the following $5,000$ draws (following~\cite{adams2010tree}).

We apply the hyperparameters: $\alpha=0.4, \gamma_0=1, \gamma=0.5, \sigma^{2}=1, L=4$.
\Cref{fg:animal} shows a rather intuitive hierarchical structure.
From the left to the right, there are insects, (potentially) aggressive mammals, herbivores, water animals, and birds.
\begin{figure}
\begin{minipage}{0.44\textwidth}
\centering
\includegraphics[scale=.45]{figures/animal_conv3}
\caption{Convergence analysis}
\label{fg:conv}
\end{minipage}
~~
\begin{minipage}{0.5\textwidth}
\centering
\includegraphics[scale=5.7]{./figures/animals_candidate_mcl_ink3.pdf}
\caption{The tree of \texttt{Animals}}
\label{fg:animal}
\end{minipage}
\end{figure}


\paragraph{\texttt{MNIST-fashion}}
This data is a collection of fashion images.
Each image is represented as a $28 \times 28$ vector of grayscale pixel values.
For better visualisation, we sample 100 samples evenly from each class.
PCA transforms the data to 22 dimensions via the asymptotic root mean square optimal threshold~\cite{Gavish2014} for keeping the singular values.
Using the same criterion as for Animal, we output two hierarchies with two sets of hyperparameters.
We set $\alpha=0.5, \gamma_0=1.5, \gamma=2, \sigma^{2}=1, L=5$.
This follows precisely the same running settings as for \texttt{Animals}.

\begin{figure*}
\centering
\includegraphics[scale=2]{./figures/mnist-fashion-mcl3}
\caption{The tree of \texttt{MNIST-fashion}}
\label{fg:fmnist}
\end{figure*}

\Cref{fg:fmnist} reflects a property of the CRP which is ``the rich get richer''.
As it is grayscale data, in addition to the shape of the items, other factors affecting the clustering might be, e.g., the foreground/background colour area, the percentage of non-black colours in the image, the darkness/lightness of the item, etc.
The hierarchical structure forms a hierarchy with high purity per level.
Some mis-labelled items are expected in a clustering task.

\paragraph{\texttt{Amazon}}
We uniformly down-sample the indices in the fashion category of \texttt{Amazon} and reserve $2,303$ entries from the data, which contain textual information about items such as their titles and descriptions\footnote{\url{http://jmcauley.ucsd.edu/data/amazon}: the data is available upon request.}.
The data is preprocessed via the method in~\cite{Gavish2014}  and only $190$ features are kept, formed as the Term Frequency and Inverse Document Frequency (TF-IDF) of the items' titles and descriptions.

In this study, we adopt a Bayesian approach to dealing with the hyperparameters.
Due to a compromise to the runtime efficiency, we run BHMC once with $500$ runs for burn-in, during which a MH-based hyperparameter sampling procedure is performed with hyperpriors $\alpha \sim \Ga(3, 1), \gamma_0 \sim \Ga(3.5, 1), \gamma \sim \U(0, 1.5)$ and $\sigma^2 \sim \U(0, 0.1)$.
We limit $\sigma^2$ as mentioned since the feature values in the data are all less than $1$ and some are far less.
In addition, $L$ is fixed to be $7$ (presuming that we have little information about the real number of levels).
The tree with the maximal complete likelihood in the subsequent $2,500$ draws is reported.

We use the evaluation methodology in~\cite{Kuang2013} to compare the clustering results against the ground-truth labels level by level.
We compare 6 levels, which is the maximum branch length of the items in the ground truth.
When extracting the labels from the trees (either for the algorithm outputs or the ground truth), items that are on a path of length less than 6 are extended to level 6 by assigning the same cluster label as that in their last level to the remaining levels.
This is to keep the consistency of the number of items for computing metrics at each level.

For the comparison, we first consider the gold standard AC with Ward distance~\cite{ward1963hierarchical}.
We adopt the existing implementations for PERCH and PYDT\footnote{\url{https://github.com/iesl/xcluster} and \url{https://github.com/davidaknowles/pydt}}.
For PYDT which is sensitive to the hyperparameters, we applied the authors' implemented hyperparameter optimisation to gather the hyperparameters prior to running the repeated simulations.
At each level, we consider four different evaluation metrics, namely, the purity, the normalised mutual information (NMI), the adjusted rand index (ARI), and the F-Measure~\cite{karypis2000comparison}.
Level 1 is the level for the root node.
% Each algorithm was repeated 35 times.
\begin{figure}[!ht]
\centering
\includegraphics[scale=.32]{./figures/amazon_after_pca-results.pdf}
\caption{Metrics on \texttt{Amazon} by levels}\label{fg:amazon-results}
\end{figure}

\Cref{fg:amazon-results} depicts that our method achieves clearly better scores with respect to purity and NMI.
In the figure, PYDT-SL and PYDT-MH correspond to the slice and the MH sampling solutions, respectively.
As the tree approaches to a lower level, our method also achieves a better performance in F-measure.
For ARI, despite that PERCH performs the best, all numerical values are exceedingly close to $0$.
However, some theoretical work of~\cite{romano2016adjusting} suggests that ARI is more preferred in the scenario that the data contains big and equal-sized clusters.
This is opposed to our ground truth which is highly unbalanced among the clusters at each level.
BHMC does show the potential to perform well according to certain traditional metrics.


==> source code/experiments_copy.tex <==
\section{Experimental Observations}
For qualitative analysis, we use the following datasets: \texttt{Compound}~\cite{ClusteringDatasets}, \texttt{Animals}~\cite{kemp2008discovery} and \texttt{MNIST-fashion}~\cite{xiao2017fmnist}.
%
%This section demonstrates  our method using the following datasets from which some qualitative analysis of the output of the method can be obtained: Compound\footnote{\url{http://cs.uef.fi/sipu/datasets/}}~\cite{ClusteringDatasets}, Animals~\cite{kemp2008discovery} and MNIST-Fashion~\cite{xiao2017fmnist}.
Following this, we carry out a quantitative analysis for the \texttt{Amazon} text data~\cite{He2016ups} since it contains the cluster labels of all the items at multiple levels.

In the following experiments, we fix $H$ to be the Normal-inverse-Wishart (NIW) distribution and unsurprisingly $F$ is set as Gaussian.
% Further, denoting the inverse Wishart with $\mathcal{W}^{-1}$, $\NIW(\nu, \lambda,  \mu_0, \Sigma_0)$ samples $\phi = (\mu, \Sigma)$ by $\mu \sim \N(\mu_0, \frac 1 {\lambda} \Sigma)$ and $\Sigma \sim \mathcal{W}^{-1}(\Sigma_0, \nu)$.
% Let $\mu_0$ and $\Sigma_0$ be fixed to the empirical mean and covariance of the data.
% We manually set $L$ for each distinct dataset.
For more complex cases, one can consider the theoretical results of the effective length of the nCRP (see Proposition 3.1 in~\cite{Steinhardt2012}).
Due to the space limit, we leave discussion of the hyperparameters for all datasets in the supplemental material.

%
% \subsection{Posterior Predictive Checking}
% For a Bayesian model, sampling from the posterior predictive distribution is a basic model check~\cite{gelman2013bayesian}.
% Before analysing the performance, we conduct this fundamental study to check if the generated data under the model look similar to the observations.
% % \begin{figure}[!ht]
% % \centering
% % \includegraphics[scale=.15]{figures/compound}
% % \caption{Compound dataset}
% % \label{fg:compound}
% % \end{figure}
% The procedure is to draw a number of random samples, after inferring the parameters of the model.
% In particular, we draw 399 (equal to the dataset size) samples from the model learned for the Compound dataset.
% In~\Cref{fg:post-checking}, there are three independent draws from the posterior. One can see that the qualitative structure of the original dataset is present in the resampled data.
% \begin{figure}[!ht]
% \centering
% \subfloat[\texttt{Compound}]{
%     \includegraphics[scale=.095]{figures/compound.pdf}
% }
% \quad
% \subfloat[Sample 1]{
%     \includegraphics[scale=.095]{figures/post_sample1.pdf}
% }
% \subfloat[Sampe 2]{
%     \includegraphics[scale=.095]{figures/post_sample2.pdf}
% }
% \quad
% \subfloat[Sample 3]{
%     \includegraphics[scale=.095]{figures/post_sample3.pdf}
% }
% \caption{Sampling from posterior distribution}
% \label{fg:post-checking}
% \end{figure}
%
% \subsection{Convergence Analysis}
% Here we examine the convergence of the algorithm using \texttt{Animals}.
% \Cref{fg:conv} shows the unnormalised log likelihood for three individual simulations.
% It is observable that they converge to a certain satisfactory level after just a few hundred runs (far less than 500).
% Although it still increases afterwards, the rate of increase becomes slower.
% \begin{figure}[ht]
% \centering
% \includegraphics[scale=.3]{figures/animal_conv}
% \caption{Convergence plots on the \texttt{Animals} dataset}
% \label{fg:conv}
% \end{figure}

\subsection{Results}
\paragraph{\texttt{Animals}}
This dataset contains 102 binary features, e.g. ``has 6 legs'', ``lives in water'', ``bad temper'', etc.
Observing the heat-map of the empirical covariance of the data, there are not many influential features.
Hence, we employ Principal Component Analysis (PCA)~\cite{murphy2012machine} to reduce it to a five-dimensional feature space.
The MCMC burns $5,000$ runs and then reports the one with the greatest complete data likelihood $p(X, \bm{c}, V \mid B, \bm{\phi}, \Theta)$ among the following $100$ draws~\cite{adams2010tree}.

\begin{figure}[ht]
\centering
\includegraphics[scale=1.9]{./figures/animals_candidate_mcl_10.eps}
\caption{The tree of \texttt{Animals}}
\label{fg:animal}
\end{figure}

In~\Cref{fg:animal}, at the first level, from left to right, we see that the first big cluster contains the bird family.
The third one contains non-insects and non-birds and is further split between the reptiles and the mammals.
They are grouped together because they have lungs and teeth and are predators; on the other hand, they share a lot of negative features: ``they have no feathers'', ``do not eat nuts'', and ``do not live in houses'', etc.
Finally, the fifth cluster contains the insects and the herbivore mammals.
Overall, the clusters separate reasonably, and the purity of the clusters is reasonably good.

\begin{figure*}
\centering
\includegraphics[scale=0.5]{./figures/mnist-fashion-mcl-5-inkscape}
% \subfloat[$\alpha=.5, \gamma_0=5, \gamma=.05, L=4, \lambda=.01, \nu=200$\label{fg:fmnist-a}]{
%   \includegraphics[scale=0.71]{./figures/mnist-fashion-mcl-5-inkscape.pdf}
% }
% \\
% \subfloat[$\alpha=.35, \gamma_0=5, \gamma=1.5, L=4, \lambda=.02, \nu=200$\label{fg:fmnist-b}]{
%   \includegraphics[scale=0.71]{./figures/mnist-fashion-mcl-4-inkscape.pdf}
% }
\caption{The tree of \texttt{MNIST-fashion}}
\label{fg:fmnist}
\end{figure*}

\paragraph{\texttt{MNIST-fashion}}
This data is a collection of fashion images.
Each image is represented as a $28 \times 28$ vector of grayscale pixel values.
For better visualisation, we sample 100 samples evenly from each class.
PCA transforms the data to 22 dimensions via the asymptotic root mean square optimal threshold~\cite{Gavish2014} for keeping the singular values.
Using the same criterion as for Animal, we output two hierarchies with two sets of hyperparameters.
We set $\alpha=0.5, \gamma_0=5, \gamma=0.05, L=4, \lambda=0.01, \nu=200$.
This executes $2,500$ burn-in runs.

% At first glance,~\Cref{fg:fmnist-a} illustrates a significant property of the CRP which is ``the rich get richer''.
% However,~\Cref{fg:fmnist-b} shows that it is also possible to have a more even grouping by changing the hyperparameters.
% As it is grayscale data, in addition to the shape of the items, other factors affecting the clustering might be, e.g., the foreground/background colour area, the percentage of non-black colours in the image, the darkness/lightness of the item, etc.
% The two hierarchies both exhibit rather reasonable structures.
% Some mislabeled items are expected in a clustering task.

\Cref{fg:fmnist} illustrates a significant property of the CRP which is ``the rich get richer''.
As it is grayscale data, in addition to the shape of the items, other factors affecting the clustering might be, e.g., the foreground/background colour area, the percentage of non-black colours in the image, the darkness/lightness of the item, etc.
The hierarchical structure forms a hierarchy with high purity per level.
Some mislabeled items are expected in a clustering task.

\paragraph{\texttt{Amazon}}
This data incorporates the information such as images, descriptions and reviews of  products in the Amazon catalogue.
We uniformly downsample the indices in the fashion category and reserve $2,303$ entries from the data, which contain textual information about items such as their titles and descriptions\footnote{\url{http://jmcauley.ucsd.edu/data/amazon}: the data is available upon request.}.
% However, the sampled identities for the data entries are providable}.
The data is preprocessed via the method in~\cite{Gavish2014}  and only $190$ features are kept, formed as the Term Frequency and Inverse Document Frequency (TF-IDF) of the items' titles and descriptions.

Our evaluation applies the methodology in~\cite{Kuang2013} to compare the clustering results against the ground-truth labels level by level.
We compare 6 levels, which is the maximum branch length of the items in the ground truth.
When extracting the labels from the trees (either for the algorithm outputs or the ground truth), items that are on a path of length less than 6 are extended to level 6 by assigning the same cluster label as that in their last level to the remaining levels up to 6.
This is to keep the consistency of the number of items for computing metrics at each level.

For the comparison, we first consider the gold standard AC with Ward distance~\cite{ward1963hierarchical}.
We adopt the existing implementations for PERCH and PYDT\footnote{\url{https://github.com/iesl/xcluster} and \url{https://github.com/davidaknowles/pydt}}.
For PYDT which is sensitive to the hyperparameters, we applied the authors' implemented hyperparameter optimisation to gather the hyperparameters prior to running the repeated simulations.
At each level, we consider four different evaluation metrics, namely, the purity, the normalised mutual information (NMI), the adjusted rand index (ARI), and the F-Measure~\cite{karypis2000comparison}.
Level 1 is the level for the root node.
Each algorithm was repeated 35 times.

\begin{figure}[!ht]
\centering
\includegraphics[scale=.32]{./figures/amazon_after_pca-results.pdf}
\caption{Metrics on \texttt{Amazon} by levels}\label{fg:amazon-results}
\end{figure}

\Cref{fg:amazon-results} is plotted with  $95\%$ confidence intervals, although the uncertainty is rather small.
It depicts that our method achieves clearly better scores with respect to purity and NMI.
In the figure, PYDT-SL and PYDT-MH correspond to the slice and the MH sampling solution, respectively.
As the tree approaches to a lower level, our method also achieves a better performance in F-measure.
For ARI, despite that PERCH performs the best, all numerical values are exceedingly close to $0$.
However, some theoretical work of~\cite{romano2016adjusting} suggests that ARI is more preferred in the scenario that the data contains big and equal-sized clusters.
This is opposed to our ground truth which is highly unbalanced among the clusters at each level.
BHMC does show the potential to perform well according to certain traditional metrics.


==> source code/hyper.tex <==
\section{Hyperparameters}
% In both sampling schemes, we can further add a Metropolis-Hastings step to update the hyperparameters.
% That is, we take advantage of the posterior $\post$ for the original tree and $\post'$ for the newly generated tree.
% It follows that we can have the acceptance rate
% \begin{align*}
% A = \min \left[1, ~\frac {\post'} {\post} \frac {q(Z \pvert Z')} {q(Z' \pvert Z)} \right] \,.
% \end{align*}
% In the sequel, the acceptance rate serves as a threshold for randomly accepting the new tree.
% In general, $q(\cdot)$ is a proposal distribution and can also be symmetric and further be canceled.

Let use denote the gamma distribution by $\Ga(\cdot)$.
We specify the hyperparameters as follows
\begin{align*}
\alpha & \sim \Ga(2, 1) \quad \gamma_0 \sim \Ga(5, 1) \quad \gamma \sim \B(2, 1) \\
L & = \ceil{l} \quad s.t.\quad l \sim \Ga(3, 0.7) + 1 \, .
\end{align*}
The distribution for the maximum levels $L$ is chosen to entail that $3$ and $4$ would appear the most frequently---we assume the most hierarchies have only three to four necessary levels.
For more complex case, one can consider the theoretical results of the effective length (see in Proposition 3.1) of nCRP in \citep{Steinhardt2012}.
Even though, the practitioners are allowed to choose their priors according to their domain knowledge about the data.

We can view the base measure $H$ as the prior to the density function $f$.
Therefore we choose a common pair as
\begin{align*}
H & = \NIW(\mu_0, \lambda, \Phi, \nu) \\
f(x \pvert \phi) &= \N(x; \mu, \Sigma) \quad i.e.~ \phi = (\mu, \Sigma) \,.
\end{align*}
$\NIW$ is the Normal-Inverse-Wishart which is usually considered the prior for a normal distribution.
We could use the empirical mean and covariance matrix of the data for $\mu_0$ and $\Phi$ respectively.
In the procedure, a covariance $\Sigma'$ for a mixture is first drawn from the inverse Wishart with the scale $1/\nu$, which means the mixture's covariance will be numerically smaller if $\nu$ is large.
Later, the mixture mean is sampled from a Gaussian such that $\mu' \sim \N(\mu, \Sigma' / \lambda)$.
For a strategy for picking the scales, we would like to see the data can be grouped into $K$ components, and hence we set the scale $\nu$ for the mixture covariance larger than $K$.
Then, we also would like to see the mixture mean across all the possible region, and thus could set $\lambda$ to satisfy   $\lambda \nu \approx 1$.

In both sampling schemes, we can further add a Metropolis-Hastings step to update the hyperparameters.
That is, we take advantage of the posterior $\post$ for the original tree and $\post'$ for the newly generated tree.


==> source code/inference.tex <==
\section{Inference}
\label{sec:inference}
We appeal to Markov Chain Monte Carlo (MCMC) for inferring the model.
One crucial property for facilitating the sampling procedure is exchangeability, which, as noted in the previous section, follows from the model's connection to the CRP.


\paragraph{Sampling $\m{V}$ and $\bm{c}$}
Following~\cite{blei2010nested}, we sample a path for a data index as a complete variable using nCRP and decide to preserve the change based on a Metropolis-Hastings (MH) step.

Recall that the component will only be drawn at the leaf.
Thus,
\begin{align}
\label{eq:update-c}
p \left(c_n = k \mid \bm{x}_n, v_{n L}=z, \m{B}, \bm{\theta}\right)
\propto
\begin{cases}
 \beta_{z k} f(\bm{x}_n; \theta_k) & \mbox{existing } k \\
 \beta^*_z f^*(\bm{x}_n) & \mbox{new } k \, .
\end{cases}
\end{align}
Sampling the set $\bm{c}$ is necessary for updating the set of mixtures at each node i.e., $\m{B}$.
Our MH scheme applies a partially collapsed Gibbs step.
Following the principles in~\cite{Dyk2015MH}, our algorithm first samples $\m{V}$ with $\bm{c}$ being collapsed out, and subsequently updates $\bm{c}$ based on $\m{V}$.


\paragraph{Sampling $\m{B}$}
It is straightforward to decide the sampling for a leaf node.
For non-root nodes, we would like to find out $p\left(c_{n} = k \mid \m{B} \setminus \{ \m{B}_{\bar{z}}\}, v_{n (L-1)} = z \right)$ where $\m{B}_{\bar{z}}$ is the set of mixing proportions in the sub-tree rooted at $z$ excluding $\bm{\beta}_z$.
% Considering $w_{z, z'} \coloneqq p\left( v_{n L} = z' \mid v_{n (L-1)} = z \right)$, we write
We write $p\left(c_{n} = k \mid \m{B} \setminus \{ \m{B}_{\bar{z}}\}, v_{n (L-1)} = z \right)$ to be
\[
p\left( v_{n L} = z' \mid v_{n (L-1)} = z \right)p\left(c_n = k \mid \bm{\beta}_{z}, v_{n L}=z', v_{n (L-1)}=z \right) \, .
\]
% \begin{align*}
% p\left(c_{n} = k \mid \m{B} \setminus \{ \m{B}_{\bar{z}}\}, v_{n (L-1)} = z \right)
% = \sum_{z'} w_{z, z'} p\left(c_n = k \mid \bm{\beta}_{z}, v_{n L}=z', v_{n (L-1)}=z \right) \, .
% \end{align*}
Logically, $p(c_n = k \mid \m{B}, \bm{v}_n) = p\left(c_n = k \mid \{\bm{\beta}_{v_{n \ell}} \}_{\ell=0}^{L} \right)$
which is then $p\left(c_n = k \mid \bm{\beta}_{v_{n L}}\right)$.
We also derive $p\left(c_n = k \mid \bm{\beta}_{z}, v_{n L}=z', v_{n (L-1)}=z \right)$ to be
\begin{align}
% \label{eq:int-over-pi}
\int p(c_n = k \mid \bm{\beta}_{z'}) d p(\bm{\beta}_{z'} \mid \bm{\beta}_{z})
&= \int p\left(c_n = k \mid \bm{\beta}_{z'} \right) \frac {\Gamma\left(\sum_{j=1}^K \gamma \beta_{z j}\right)} {\prod_{j=1}^K \Gamma(\gamma \beta_{z j})} \prod_{j=1}^K \beta_{z' k}^{\gamma \beta_{z k} - 1} d \bm{\beta}_{z'} \nonumber \\
&= \frac {\Gamma\left(\sum_{j=1}^K \gamma \beta_{z j}\right)} {\prod_{j=1}^K \Gamma(\gamma \beta_{z j})} \int \prod_{j=1}^K \beta_{z' j}^{\mathds{1}\{c_{n} = k\} + \gamma \beta_{z k} - 1} d \bm{\beta}_{z'} \nonumber \\
&= \frac {\Gamma\left(\sum_{j=1}^K \gamma \beta_{z j}\right)} {\prod_{j=1}^K \Gamma(\gamma \beta_{z j})} \frac {\prod_{j=1}^K \Gamma(\mathds{1}\{c_{n} = k\} + \gamma \beta_{z j})} {\Gamma(1 + \sum_{j=1}^K \gamma \beta_{z j})} = \beta_{z k} \nonumber \,
\end{align}
given that $\Gamma(x + 1) = x \Gamma(x)$ holds when $x$ is any complex number except the non-positive integers.
% Full derivation details are displayed in the supplemental material.
Therefore, $p\left(c_{n} = k \mid \m{B} \setminus \{ \m{B}_{\bar{z}}\}, v_{n (L-1)} = z \right)=\beta_{z k}$.
This indicates that, marginalising out the subtree rooted at $z$, the component assignment is thought to be drawn from $\bm{\beta}_{z}$, which can be seen through induction.
Therefore, it allows us to conduct the size-biased permutation,
\begin{align}
\mbox{root } z_0 & &\beta_{z_0 1}, \dots, \beta_{z_0 K}, \beta_{z_0}^* &\sim \Dir\left(N_{z_0 1}, \dots, N_{z_0 K}, \gamma_0 \right) \label{eq:update-b-root} \\
\forall z': (z, z') \in \eset & & {\beta}_{z'1}, \dots, \beta_{z'K}, \beta^*_{z'} &\sim \Dir\left({\tilde N}_{z'1}, \dots, {\tilde N}_{z'K}, \gamma \beta^*_{z} \right) \label{eq:update-b}
\end{align}
where $\tilde{N}_{z' k} = N_{z'k} + \gamma \beta_{z k}$.
\Cref{eq:update-b-root} employs a Poly\'{a} urn posterior construction of the DP to preserve the exchangeability when carrying out the size-biased permutation~\cite{pitman1996some}.
% \begin{align}
% \beta_{z_0 1}, \dots, \beta_{z_0 K}, \beta_{z_0}^* &\sim \Dir\left(N_{z_0 1}, \dots, N_{z_0 K}, \gamma_0 \right) \, . \label{eq:update-b-root}
% \end{align}
% Then, for each $z'$ such that $(z, z') \in E_V$, assuming $\tilde{N}_{z' k} = N_{z'k} + \gamma \beta_{z k}$, we write
% \begin{align}
%  {\beta}_{z'1}, \dots, \beta_{z'k}, \beta^*_{z'} &\sim \Dir\left(\tilde{N}_{z'1} , \dots, \tilde{N}_{z'k}, \gamma \beta^*_{z} \right)  \label{eq:update-b} \, .
% \end{align}
% \Cref{eq:update-b-root} employs a Poly\'{a} urn posterior construction of the DP to preserve the exchangeability when carrying out the size-biased permutation~\cite{pitman1996some}.
This step in our inference enables an analytical form of node parameter update.

% \paragraph{Sampling $\bm{\theta}$}
% We write, given $p(\theta_k \mid \data, \bm{c}, H)
% \sim p(\theta_k \mid H) p(\data \mid \bm{c}, \theta_k, H)$,
% \begin{align}
% \label{eq:update-par}
% p(\theta_k \mid \data, \bm{c}, H)
% &\sim p(\theta_k \mid H) \prod_{n: c_n=k} p(\bm{x}_n \mid \theta_k) \,.
% \end{align}
% The principle for a conditional sampling for DP is to sample a sufficiently large (but finite) number of samples.
% Hence, more $\theta$'s than $K$ will be sampled always.



\paragraph{Sampling $\bm{\theta}$}
Even though there are many options for $H$, we choose a Gaussian distribution in this paper.
With $\theta_k \coloneqq \bm{\mu}_k$,
%Here, $H$ samples the mean, $\mu$, for $F$ which is also a Gaussian distribution with known covariance matrix $\m{\Sigma}$.
%More specifically, $\theta_k \coloneqq \bm{\mu}_k$.
we define $f(\bm{x}; \bm{\mu}_k) = \N(\bm{x}; \bm{\mu}_k, \m{\Sigma})$ and $H = \N(\bm{\mu}_0, \m{\Sigma}_0)$, where covariance matrices $\m{\Sigma}$ and $\m{\Sigma}_0$ are known and fixed.
Collapsing out the unused terms, we can write
$p(\theta_k \mid \data, \bm{c}) \sim p(\theta_k \mid H) \prod_{n: c_n=k} p(\bm{x}_n \mid \theta_k) \,.$
Given the conjugacy of a Gaussian prior with a Gaussian of known covariance,
% \begin{equation}
% \label{eq:update-phi}
% \bm{\mu}_k \mid \data, \bm{c} \sim \N(\tilde{\bm{\mu}}_k, \tilde{\m{\Sigma}}_k)
% \end{equation}
% where,
by considering $\bar{\bm{x}}_k = \frac 1 {N_k} \sum_{n} \mathds{1}\{c_n = k\} \bm{x}_n$ and $N_K = \sum_n \mathds{1}\{c_n = k\}$,
we obtain $\bm{\mu}_k \mid \data, \bm{c} \sim \N(\tilde{\bm{\mu}}_k, \tilde{\m{\Sigma}}_k)$ where
\begin{align}
  \label{eq:update-phi}
  \tilde{\bm{\mu}}_k = \tilde{\m{\Sigma}}_k (\m{\Sigma}_0^{-1} \bm{\mu}_0 + N_k \m{\Sigma}^{-1} \bar{\bm{x}}_k)
  \qquad
  \tilde{\m{\Sigma}}_k = (\m{\Sigma}_0^{-1} + N_k \m{\Sigma}^{-1})^{-1} \, .
\end{align}
% \begin{align}
%   \label{eq:update-phi}
%   &\bm{\mu}_k \mid \data, \bm{c} \sim \N(\tilde{\bm{\mu}}_k, \tilde{\m{\Sigma}}_k) \nonumber \\
%   \mbox{where \quad } &\tilde{\bm{\mu}}_k = \tilde{\m{\Sigma}}_k (\m{\Sigma}_0^{-1} \bm{\mu}_0 + N_k \m{\Sigma}^{-1} \bar{\bm{x}}_k)
%   \qquad
%   \tilde{\m{\Sigma}}_k = (\m{\Sigma}_0^{-1} + N_k \m{\Sigma}^{-1})^{-1} \, .
% \end{align}


\subsection{Algorithmic Procedure}
In practice, one useful step of the inference is to truncate the infinite setting of $\bm{\beta}_{z_0}$ to a finite setting.
Referring back to~\Cref{eq:lkhd}, one can have a threshold such that the sampling of $\bm{\beta}_{z_0}$ terminates when the remaining length of the stick $\beta_{z_0}^*$ is shorter than that threshold.
% It is worth noting that, choosing $H$ to be a conjugate prior of $F$ makes $f^*(x)$ trivially computable.
Once a new component is initialised, each node will update its $\bm{\beta}$ by one more stick-breaking step.
That is, for the root node, it samples one $u$ from $\B(1, \gamma_0)$, and assigns $\beta_{{z_0} (K+1)} = \beta_{z_0}^* u$ and the remaining stick length $1-\sum_{k=1}^{K+1} \beta_{{z_0} k}$ as a new $\beta_{z_0}^*$.
For a non-root node $z'$ inheriting from node $z$, we apply the results from the preliminary section such that $u$ is sampled from $\B(\gamma \beta_{z (K+1)}, \gamma \beta_{z}^*)$ and then update in the same manner as the root node.
% Finally, set $K \gets K+1$.

% \begin{align}
% \label{eq:update-phi}
% \bm{\mu}_k \sim \N\left((\m{\Sigma}_0^{-1} + N_k \m{\Sigma}^{-1})^{-1}(\m{\Sigma}_0^{-1} \bm{\mu}_0 + N_k \m{\Sigma}^{-1} \bar{\bm{x}}_k), (\m{\Sigma}_0^{-1} + N_k \m{\Sigma}^{-1})^{-1} \right)
% \end{align}
% where $\bar{\bm{x}}_k = \frac 1 {N_k} \sum_{n:c_n=k} \bm{x}_n$ and $N_K = \sum_n \mathds{1}(c_n = k)$.

% Thus, a reasonable value of the initial threshold for cutting the mixing proportions is flexible and will not violate the infinite configuration, while setting a better threshold does improve runtime efficiency by reducing the adjustments and updates for drawing a new component.

\Cref{alg:scheme-a} depicts the procedure.
The MH scheme samples a proposal path and the corresponding $\bm{\beta}$'s if new nodes are initialised.
MH considers an acceptance variable $\mathcal{A}$ such that $\mathcal{A}
= \min \left\{1, \frac {\post' q(\m{V}, \m{B} \mid \m{V}', \m{B}')} {\post q(\m{V}', \m{B}' \mid \m{V}, \m{B})} \right\}$.
Here, $\post$ and $\post'$ are the posteriors at the current and proposed states, respectively.
Then, $q$ is the proposal for sampling $\m{V}'$ and $\m{B}'$, which in our case is the nCRP and HDP.
At each iteration for a certain data index $n$, $\m{V}$ changes to $\m{V}'$ by replacing $\bm{v}_n$ with $\bm{v}'_n$.
Thus, in this example, $q(\m{V}' \mid \m{V}) = \ncrp(\bm{v}'_n; \m{V} \setminus \{\bm{v}_n\})$ and vice versa.
The term $q(\m{B} \mid \m{V}) / q(\m{B}' \mid \m{V}')$ is cancelled out by the terms $p(\m{B}' \mid \m{V}') / p(\m{B} \mid \m{V})$ in the posterior, as $q(\m{B} \mid \m{V})$ and $p(\m{B} \mid \m{V})$ are identical.
Apart from that, $\bm{\theta}$ will be updated only after all the paths are decided, and hence gain no changes.
Therefore, for a specific $\bm{x}_n$, we have that
\begin{align*}
\mathcal{A} =
\min \left\{1,~ \frac {p(\bm{x}_n \mid \beta_{v'_{n L}}, v'_{n L}, \bm{\theta}) p(\m{V}') } {p(\bm{x}_n \mid \beta_{v_{n L}}, v_{n L}, \bm{\theta}) p(\m{V})} \frac {\ncrp(\bm{v}_n; \m{V}' \setminus \{\bm{v}'_n\})} {\ncrp(\bm{v}'_n; \m{V} \setminus \{\bm{v}_n\})} \right\}
\end{align*}
given that the likelihood for $\data \setminus \{\bm{x}_n\}$ remains unaltered.
After the paths $\m{V}$ for all the observations are sampled, the process updates $\m{B}$ and $\bm{\theta}$ using the manner discussed above.


\subsection{Time Complexity}
Contrary to first impression, at each iteration, the algorithm complexity is only $N^2$ for the worst case, and log-linear for the expected case.

% \begin{lemma}
% The worst complexity of the MH sampler for each iteration is $O(N^2(L+ g_s(D)))$ where $g_s(D)$ is the complexity of sampling a $D$-dimensional mean vector using the Gaussian prior.
% In addition, the average case complexity is bounded by $O(N\log N (L + g_s(D)))$.
% \end{lemma}
% \begin{proof}
Assume that the maximum number of children is $M_{z_\ell}^*$ at the level $\ell$, then the cost of sampling a path for a single observation with the nCRP is $O (\sum_{\ell=1}^L M^*_{z_\ell} )$.
After that, sampling $c_n$ is carried out with time $O(K g(D))$ where $g(D)$ is the time for computing the Gaussian likelihood of $D$-dimensional data.
%Here, we finish the global variables.
In regard to the global variables, $\m{B}$ will be updated with every node and thus achieves $O(K \lvert \nset \rvert)$.
Lastly, $\bm{\theta}$ will be updated with time $O(K g_s(D))$ where $g_s(D)$ is the complexity of sampling the Gaussian mean.
In addition, we notice $\sum_{\ell=1}^L M^*_{z_\ell} = O(\lvert \nset \rvert)$ and $g(D) = O(g_s(D))$.
Overall, for one iteration, we can summarise the complexity by
$
\textstyle  N \sum_{\ell=1}^L M^*_{z_\ell} + K \lvert \nset \rvert + N K g_s(D) = O((N + K) \lvert \nset \rvert + N K g_s(D)) \, .
$
Since the number of components will not exceed the data size, $K \le N$ holds.
With respect to $\lvert \nset \rvert$, at each level, it is no more than $N$.
The extreme case is that each datum is a node and extends to $L$ levels.
It follows that $\lvert \nset \rvert \le NL$.
Hence, $O((N + K) \lvert \nset \rvert + N K g_s(D)) = O \left(N^2 (L + g_s(D)) \right)$.

The expected number of DP components, considering $\gamma_0$, is $\gamma_0 \log N$ for sufficiently large $N$~\cite{murphy2012machine}. Likewise for the first level in the nCRP, which is then $\alpha \log N$.
Let $\E[\cdot]$ denote the expectation over all random $\tree$ drawn from the BHMC. %be short for $\E_{\tree \sim \mbox{BHMC}}[\cdot]$.
If $N$ is sufficiently large, we can have $\sum_{\ell=1}^L \E [M_{z_\ell}] = O(L\alpha \log N)$, %with the maximum number $M^*$ being replaced by a random $M$,
as the expected number of nodes will be no greater than $\alpha \log N$.
However, $\E [\lvert \nset \rvert]$ is hard to decide but is known to be $\le \min(NL, (\alpha \log N)^L)$.
If $N \gg 0$ and $\alpha > 0$, then $NL \le (\alpha \log N)^L$.
% Otherwise, if $\alpha$ is arbitrarily small, there will be always one node under a parent, so that $\lvert \nset \rvert = L$.
% \begin{align*}
% N (\sum_{\ell=1}^L \E [M_z] + \E[K] g_s(D)) + \E[K \lvert \nset \rvert]
% &= O(N \log N (\alpha L + \gamma_0 g_s(D)) + \gamma_0 \log N \lvert \nset \rvert) \\
% &= O(N \log N (\alpha L + \gamma_0 g_s(D)) + \gamma_0 N L \log N ) \\
% &= O(N \log N (2 L + g_s(D))) \,.
% \end{align*}
We can obtain $N (\sum_{\ell=1}^L \E [M_z] + \E [K] g_s(D)) = O(N \log N (\alpha L + \gamma_0 g_s(D)))$ and $\E [K \lvert \nset \rvert] = O(\gamma_0 \log N \times N L)$.
Combining the two expressions, we derive the upper bound $O(N \log N (L + g_s(D)))$ for the average case.
% \qed
% \end{proof}


==> source code/intro.tex <==
\section{Introduction}
We study the problem of Hierarchical Clustering (HC) via a Bayesian Nonparametric (BNP) modelling perspective.
A BNP proposes a generative model for the observed data whose dimension is not fixed, but rather is learned from the data. In the case of HC, this allows the structure of the hierarchy to be inferred along with its clusters.
Considering a model for generating the data, a BNP for HC typically associates each node in the hierarchy with a particular choice of parameters.
Then the model consists of two components: 1) the random process for generating a path through the hierarchy from the root node to a leaf; 2) a parent-to-child transition kernel that models how  a child node's parameters are related to those of its parent.
The generative model posits that each observation firstly selects a path randomly, and is then sampled through the distribution associated with the leaf node of the path.
\begin{figure}
\centering
\subfloat[Gaussian node \label{fg:gauss-node}]{
  \includegraphics[scale=0.21]{figures/mm2}
}
~
\subfloat[Mixture node \label{fg:mixture-node}]{
  \includegraphics[scale=0.21]{figures/mm1}
}
\caption{A simple example of the two nodes (distinguished by colour) at the first layer after the root node.~\Cref{fg:gauss-node} depicts a manner of clustering the data with Gaussian-to-Gaussian node transition from root to the level 1, and~\Cref{fg:mixture-node} is the version of applying HDPMM.}
\label{fg:kernel-comparison}
\end{figure}

An early example of the parametric generative probabilistic model is the Gaussian tree generative process~\cite{williams2000mcmc}, such that each non-root node is sampled from a Gaussian distribution with the mean of the parent node and predefined level-wise covariances.
In general, for the first component, there are some well-known random processes, e.g. the nested Chinese Restaurant Process (nCRP)~\cite{blei2010nested,adams2010tree}, the Dirichlet Diffusion Tree (DTT)~\cite{neal2003density}, the Pitman-Yor Diffusion Tree (PYDT)~\cite{Knowles2015}, which is a generalisation of the DTT, and the  tree-structured stick-breaking construction (TSSB)~\cite{adams2010tree}, which generalises  the (nCRP).
It is proved in~\cite{Knowles2015}, that the nCRP and PYDT (and so also the DTT) are asymptotically equivalent---thus, this work focuses on the second component and selects the nCRP for the first component, given its simplicity.
Existing BNP methods mostly utilise Gaussian-to-Gaussian (G2G) diffusion kernels for the node parameters~\cite{neal2003density,williams2000mcmc,adams2010tree,Knowles2015}.
Within such a setting, e.g., if a parent node's distribution is (denoted by $\sim$) $\N(\bm{\mu}_p, \m{\Sigma}_p)$, its child has the node parameters $\bm{\mu}_c \sim \N(\bm{\mu}_p, \m{\Sigma}_p)$ and is associated with the data distribution $\N(\bm{\mu}_c, \m{\Sigma}_c)$ where $\m{\Sigma}_p$ and $\m{\Sigma}_c$ can be predefined hyperparameters.

G2G kernels are easy to apply but somehow lack the ability to handle more complex patterns.
In our work, we investigate the Hierarchical Dirichlet Process Mixture Model (HDPMM) for the parent-to-node transition.
In this setting, each node is actually a mixture distribution and the node parameters maintain the mixture weights for a global book of components.
Then, the parent-to-node transition follows a Hierarchical Dirichlet Process (HDP)~\cite{teh2010hierarchical}. As a simple example, in~\Cref{fg:kernel-comparison}, a single level of clustering is applied to the shown data points, using G2G~(\Cref{fg:gauss-node}) and HDPMM~(\Cref{fg:mixture-node}). The HDPMM fits a mixture model to the purple nodes, which can be further refined in lower levels of the tree.
Note that, the HDP~\cite{Teh2006hier} is discussed in~\cite{adams2010tree}, for applications based on Latent Dirichlet Allocations.
However, our setting HDPMM is more suited to general clustering.

% {\bf Our contributions} are three-fold: 1) we present a Bayesian Nonparametric model for Bayesian Hierarchical Mixture Clustering thoroughly; 2) we show that the computational time is polynomial; 3) we empirically demonstrate the performance of the algorithm, showing that it outperforms a number of other HC methods according to some standard clustering metrics.


\subsubsection{Related work}
Our focus is on statistical methods, despite that there are many non-statistical methods for HC e.g. \cite{ward1963hierarchical,Monath2019,kobren2017hierarchical,charikar2019hierarchical}, to name just a few.
Statistical extensions to Agglomerative clustering (AC) have been proposed in~\cite{stolcke1993hidden,iwayama1995hierarchical,heller2005bhc,lee2015bayesian} but these are not generative models.
On the other hand, Teh et al.~\cite{teh2008bayesian} has proposed applying the Kingman's coalescent as a prior to the HC, which is similar in spirit to DDT and PYDT, however it is a backward generative process.

It is worth mentioning that the tree generation and transition kernels that we exploit have been used in a number of other contexts, beyond HC. For example, Paisley et al.~\cite{paisley2015nested} discuss the nested Hierarchical Dirichlet Process (nHDP) for topic modelling which, similar to the method we present here, uses the nCRP to navigate through the hierarchy, but associates nodes in the tree with topics. The nHDP first generates a global topic tree using the nCRP where each node relates to one atom (topic) drawn from the base distribution. In summary, nHDP constitutes multiple trees with one global tree and many local trees, whereas our construction has a single tree capturing the hierarchical structure of the data. Ahmed et al.~\cite{Ahmed2013} also proposed a model that is very similar to the nHDP, but appealed to different inference procedures.


==> source code/model.tex <==
\section{Generative Process}
We call our model BHMC, for Bayesian Hierarchical Mixture Clustering and illustrate it using \Cref{fg:tree-example}.

\begin{wrapfigure}{r}{0.4\textwidth}
 \centering
 \scalebox{0.5}{
 \begin{forest}
   for tree={
     circle, draw, very thick, edge={very thick}
   }
   [$\bm{\beta}_{z_0} $
     [$\bm{\beta}_{z_1}$, edge label={node[midway,left]{$w_{z_0 1}$}}
       [$\bm{\beta}_{z_3} $, edge label={node[midway,left]{$w_{z_1 1}$}}]
       [$\bm{\beta}_{z_4} $, edge label={node[midway,right]{$w_{z_1 2}$}}]
     ]
     [$\bm{\beta}_{z_2} $, edge label={node[midway,right]{$w_{z_0 2}$}}
       [$\bm{\beta}_{z_5} $]
       [$\bm{\beta}_{z_6} $]
       [$\bm{\beta}_{z_7} $]
     ]
   ]
 \end{forest}
 }
 \caption{One example of a BHMC hierarchy}
 \label{fg:tree-example}
 \vspace{-10pt}
\end{wrapfigure}

\iffalse
We propose a ``Chinese Hierarchical Restaurant Franchise'' (CHRF) metaphor to motivate our generative process. This metaphor extends the Chinese Franchise metaphor proposed in~\cite{Teh2006hier}, to multilevel hierarchical arrangements and combines with the nCRP to choose a path in this hierarchy.  Note that this is distinct from the nested Chinese Restaurant Franchise (nCRF) proposed in~\cite{Ahmed2013} for topic modelling. In common with the nCRF, our process uses the nCRP to generate the hierarchical structure, but our process for generating observations is different, as we rely on a multilevel HDP to connect mixture components along an L-level path in the tree, while, in the nCRF, corresponding nodes in a global and local tree are connected through a single level HDP.
Check supplemental material for a detailed description of the metaphor summarised below.
\fi

Let $z$ be the label for a certain node in the tree.
We can denote the probability to choose the first child under $z$ by $w_{z 1}$.
Also, let us denote the mixing proportion for a node $z$ by $\bm{\beta}_z$, and denote the global component assignment for the $n^{th}$ data item, $\bm{x}_n$, by $c_n$. To draw $\bm{x}_n$, the hierarchy is traversed to a leaf node, $z$, at which $c_n$ is drawn from mixing proportions $\bm{\beta}_z$.
A path through the hierarchy is denoted by a vector e.g. $\bm{v} = \{z_0, z_1, z_4\}$.
In a finite setting, with a fixed number of branches, such a path would be generated by sampling from weights $\bm{w}_{z_0} \sim \Dir(\alpha)$, at the first level, then $\bm{w}_{z_1} \sim \Dir(\alpha)$ at the second level and so on. The nCRP enables the path to be sampled from infinitely branched nodes.
Mixing proportions, $\bm{\beta}_z$, along a path are connected via a multilevel HDP. Hence, if the probability of a mixture component goes to zero at any node in the tree, it will remain zero for any descendant nodes. Moreover, the smaller $\gamma$ is, the sparser the resulting distribution drawn from the HDP~\cite{murphy2012machine}.
% Fewer and fewer mixture components are possible when draws are made from proportions associated with deeper levels of the tree.

The generative process with an infinite configuration is shown in~\Cref{alg:generative}.
For a finite setting, the mixing proportions are on a finite set and Line~1 should be changed to $\bm{\beta}_{z_0} \sim \Dir(\gamma_0/K, \dots, \gamma_0/K)$.
Correspondingly, Line 9 has to be changed to $\bm{\beta}_{z'} \sim \Dir(\gamma \bm{\beta}_z)$ according to the preliminary section.
%
% \begin{algorithm}
% \LinesNumbered
% \SetAlgoVlined
% \DontPrintSemicolon
% \caption{Generative process (infinite)}\label{alg:generative}
% Sample $\bm{\beta}_{z_0} \sim \Gem(\gamma_0)$ \label{GPalgo:infi:root}\\
% Sample $\theta_1, \theta_2, \theta_3, \dots \sim H$ \\
% \For{$n=1 \dots N$}{
%   $v_n^0 \gets z_0$ \\
%   \For{$\ell = 1 \dots L$} {
%     Sample $v^{\ell}_n$ using CRP($\alpha$) \\
%     $z \gets v_n^{\ell-1}$, $z' \gets v_{n \ell}$ \\
%     \If{$z'$ is new}{
%       Sample $\bm{\beta}_{z'} \sim \DP\left(\gamma, \bm{\beta}_{z}\right)$ \label{GPalgo:infi:nonroot} \\
%       Attach $(z, z')$ to the tree
%     }
%   }
%   Sample $c_n \sim \D\left(\bm{\beta}_{v_{n L}}\right)$ \\
%   Sample $\bm{x}_n \sim F(\theta_{c_n})$
% }
% \end{algorithm}

% \begin{algorithm}[!ht]
% \caption{Generative process (infinite)} \label{alg:generative}
% \begin{algorithmic}[1]
% \STATE \label{GPalgo:infi:root} Sample $\bm{\beta}_{z_0} \sim \Gem(\gamma_0)$
% \STATE Sample $\theta_1, \theta_2, \theta_3, \dots \sim H$
% \FOR{$n=1 \dots N$}
%   \STATE $v_n^0 \gets z_0$
%   \FOR{$\ell = 1 \dots L$}
%     \STATE Sample $v^{\ell}_n$ using CRP($\alpha$)
%     \STATE $z \gets v_n^{\ell-1}$, $z' \gets v_{n \ell}$
%     \IF{$z'$ is new}
%       \STATE Sample $\bm{\beta}_{z'} \sim \DP\left(\gamma, \bm{\beta}_{z}\right)$ \label{GPalgo:infi:nonroot}
%       \STATE Attach $(z, z')$ to the tree
%     \ENDIF
%   \ENDFOR
%   \STATE Sample $c_n \sim \D\left(\bm{\beta}_{v_{n L}}\right)$
%   \STATE Sample $\bm{x}_n \sim F(\theta_{c_n})$
% \ENDFOR
% \end{algorithmic}
% \end{algorithm}

\subsection{Properties}
Let us denote the tree by $\tree = (\nset, \eset)$.
First, the node set is $\nset=\{z_0, \dots, z_{M-1}\}$ where $M$ is the number of nodes.
Then, $\eset$ is the set of edges in the tree, where $(z,z') \in \eset$ means that there exists some path $\bm{v}_n$, such that $\bm{x}_n$ moves from $z$ to $z'$ in the path $\bm{v}_n$.
Hence, we infer the following variables:
$\m{B} = \{\bm{\beta}_{z_0}, \dots, \bm{\beta}_{z_{M-1}}\}$, the mixing proportions for the components in the node $z$;
$\bm{\theta}=\{\theta_1, \dots, \theta_K\}$, component parameters;
$\m{V} = \{\bm{v}_1, \dots, \bm{v}_N \}$ where each $\bm{v}_n = \{v_{n 0}, v_{n 1}, \ldots, v_{n L}\}$ is the ordered set of nodes in $\nset$ corresponding to the path of $\bm{x}_n$;
$\bm{c} = \{c_1, \dots, c_N\}$, the component label for all the observations.
% \begin{itemize}
% \item
% $\m{B} = \{\bm{\beta}_{z_0}, \dots, \bm{\beta}_{z_{M-1}}\}$, the mixing proportions for the components in the node $z$
% \item
% $\bm{\theta}=\{\theta_1, \dots, \theta_K\}$, component parameters
% \item
% $\m{V} = \{\bm{v}_1, \dots, \bm{v}_N \}$ where each $\bm{v}_n = \{v_{n 0}, v_{n 1}, \ldots, v_{n L}\}$ is the ordered set of nodes in $\nset$ corresponding to the path of $\bm{x}_n$
% \item
% $\bm{c} = \{c_1, \dots, c_N\}$, the component label for all the observations
% \end{itemize}
Denoting $\Phi = \{{\gamma_0}, \gamma, \alpha, H, L\}$, we focus on the marginal prior $p(\m{V}, \bm{\theta}, \m{B} \mid \Phi)$ and obtain $p(\m{V}, \bm{\theta}, \m{B} \mid \Phi) = p(\m{B} \mid \m{V}, \gamma_0, \gamma) p(\m{V} \mid \alpha, L) p(\bm{\theta} \mid H)$.

The first term is $p(\m{B} \mid \m{V}, \gamma_0, \gamma) = p\left(\bm{\beta}_0 \mid {\gamma_0}\right)\prod_{(z, z') \in \eset} p(\bm{\beta}_{z'} \mid \gamma, \bm{\beta}_{z})$.
To expand the second term, we first denote by $m_{z}$ the number of children of $z$.
Hence, the CRP probability for a set of clusters $\{z'_{n}\}_{n=1}^{m_z}$ under the same parent $z$~\cite{ferguson1973bayesian,antoniak1974mixtures}:
\[
p(\{z'_{n}\}_{n=1}^{m_z} \mid \alpha) = \frac {\alpha^{m_z} \Gamma(\alpha)} {\Gamma(N_{z} + \alpha)} \prod_{n=1}^{m_z} \Gamma\left(N_{z'_n}\right)
\]
where $N_z$ is the number of observations in $z$.
With this equation, one can observe the exchangeability of the order of arriving customers---the probability of obtaining such a partition is not dependent on the order.
The tree $\tree$ is constructed via $\m{V}$ with the empty nodes all removed.
For such a tree, the above result can be extended to
\[
\textstyle
p(\m{V} \mid \alpha)
= \Gamma(\alpha)^{\lvert \mathcal{I}_{\tree} \rvert}\prod_{z \in \mathcal{I}_{\tree}} \frac {\alpha^{m_{z}}} {\Gamma(N_{z}+\alpha)} \prod_{(z, z') \in \eset} \Gamma(N_{z'})
\]
where $\mathcal{I}_{\tree}$ is the set of internal nodes in $\tree$.
Next, we obtain $p(\bm{\theta} \mid H) = \prod_{k=1}^K p(\theta_k \mid H)$.
% Considering the marginal likelihood $p(\bm{x}_n \mid V, \bm{\theta}, \m{B})$ is actually $p(\bm{x}_n \mid v_{n L}=z, \bm{\theta}, \bm{\beta}_{z})$, the likelihood for a single observation is
% \begin{align}
% p(\data \mid V, \bm{\theta}, B)
% &= \prod_{i=1}^{N}\sum_{k=1}^K  p\left(\bm{x}_n, c_n=k \mid v_{n L}=z, \bm{\theta}, \bm{\beta}_{z}\right) = \prod_{i=1}^{N}\sum_{k=1}^K \beta_{z k} f(\bm{x}_n; \theta_k) + \beta_z^* f^*(x)
% \end{align}
The likelihood for a single observation  is
\begin{equation}
\label{eq:lkhd}
\textstyle p\left(\bm{x}_n \mid v_{n L}, \bm{\theta}, \bm{\beta}_{v_{n L}}\right) =
 \sum_{k=1}^K \beta_{v_{n L} k} f(\bm{x}_n; \theta_k) + \beta_{v_{n L}}^* f^*(\bm{x}_n)
\end{equation}
where $\beta^*_{z}$ denotes the probability of drawing a new component which is always the last element in the vector $\bm{\beta}_z$.
Here, $f(\cdot)$ is the corresponding density function for the distribution $F$ and we obtain $f(\bm{x}; \theta) \equiv p(\bm{x} \mid \theta)$.
Furthermore, $f^*(\bm{x}) = \int p(\bm{x} \mid \theta) d p(\theta \mid H)$.
The above presentation is similar to the Poly\'{a} urn construction of DP~\cite{pitman1996some}, which trims the infinite setting of DP to a finite configuration.
Then, one can see $ p(\data \mid \m{V}, \bm{\theta}, \m{B}) = \prod_{n} p\left(\bm{x}_n \mid v_{n L}, \bm{\theta}, \bm{\beta}_{v_{n L}}\right)$.
Finally, the unnormalised posterior is
$
p(\m{V}, \bm{\theta}, \m{B} \mid \data, \Phi) \propto p(\data \mid \m{V}, \bm{\theta}, \m{B}) p(\m{V}, \bm{\theta}, \m{B} \mid \Phi)
$.

\hspace{-4ex}
\begin{minipage}{.54\textwidth}
\begin{algorithm}[H]
\DontPrintSemicolon
\caption{Generative process (infinite)}\label{alg:generative}
Sample $\bm{\beta}_{z_0} \sim \Gem(\gamma_0)$ \label{GPalgo:infi:root}\\
Sample $\theta_1, \theta_2, \ldots \sim H$ \\
\For{$n=1 \dots N$}{
  $v_{n 0} \gets z_0$ \\
  \For{$\ell = 1 \dots L$} {
    Sample $v_{n \ell}$ using CRP($\alpha$) \\
    $z, z' \gets v_{n (\ell-1)}, v_{n \ell}$ \\
    \If{$z'$ is new}{
      Sample $\bm{\beta}_{z'} \sim \DP\left(\gamma, \bm{\beta}_{z}\right)$ \label{GPalgo:infi:nonroot}\\
      Attach $(z, z')$ to the tree
    }
  }
  Sample $c_n \sim \Cat\left({\beta}_{v_{n L}}\right)$ \\
  Sample $\bm{x}_n \sim F(\theta_{c_n})$ \\
}
\end{algorithm}
\end{minipage}
~
\begin{minipage}{.45\textwidth}
\begin{algorithm}[H]
\DontPrintSemicolon
\caption{MH sampler}\label{alg:scheme-a}
\tcp{$\epsilon$: stopping threshold}
Sample $\bm{\beta}_{z_0}$ until $\beta^*_{z_0} < \epsilon$ \\% arbitrarily small value \\
\For{$\bm{x}_n \in \textsc{Shuffled}(\data)$}{
  Clean up $c_n$ and $\bm{v}_n$ \\
  Sample $\hat{\bm{v}}_n$ (and possibly new $\bm{\beta}$) through the generative process \\
  $s \sim \U(0, 1)$ \\
  \lIf{$s \le \mathcal{A}$}{
    $\bm{v}_n \gets \hat{\bm{v}}_n$
  }
  Sample ${c}_n$ using a Gibbs step by~\Cref{eq:update-c}
}
Update $\m{B}$ by~\Cref{eq:update-b-root,eq:update-b} \\
Update ${\bm{\theta}}$ by~\Cref{eq:update-phi}
\end{algorithm}
\end{minipage}%


==> source code/preliminary.tex <==
% \section{Preliminary}
% % We present a mixture model of the data, whose parameters are selected from a hierarchy (or tree).
% Our model will make heavy use of knowledge of the Dirichlet Process (DP) and the Hierarchical Dirichlet Process (HDP), which are summarised next.
% This section introduces the related knowledge.
%
%
% \subsection{Hierarchical Mixture Model}
% \label{sec:hiermixmodel}
% A mixture model for a set of $N$ data items $\{\bm{x}_n\}_{n=1}^N$ over $K>0$ mixture components firstly generates a set of $K$ parameters $\theta_k$, from a base distribution $H$.
% Then, for each data point $\bm{x}_n$, it randomly chooses a component $c_n$ according to the mixture proportions $\bm{\beta}$ and generates $\bm{x}_n$ from a distribution $F(\cdot)$ depending on the parameters $\theta_{c_n}$:
% \begin{align}
% \label{eqn:mixturemodel}
% \{\beta_k\}_{k=1}^K &\sim \Dir(\alpha/K, \dots, \alpha/K) \quad  & c_n &\sim \D(\bm{\beta})  \nonumber\\
% \{\theta_k\}_{k=1}^K  &\sim H\quad & \bm{x}_n  &\sim F(\theta_{c_n}) \, .
% \end{align}
% We consider a hierarchy, such that each node in the tree is associated with a particular mixture distribution $\bm{\beta}$.  A hierarchical mixture model is formed by, for each data point, navigating through the tree to a particular node, $z$, choosing the mixture proportions $\bm{\beta}_z$ associated with that node and generating the data point according to Equation ~\eqref{eqn:mixturemodel}.
% Let $z'$ be a child of $z$ in the hierarchy. We connect the mixture proportions along a path in the tree through the relationship ${\bm{\beta}}_{z'} \sim \Dir(\gamma \bm{ \beta}_z)$
% for concentration parameter $\gamma>0$. Hence the mixture proportions of the desecendant nodes along any path have the same expected value as the parent, but tend to become more concentrated as the length of the path increases.
% We extend this idea to allow for an infinite number of components.
% Therefore, before elaborating on our idea, it is necessary to introduce the Dirichlet Process (DP) and the Hierarchical Dirichlet Process (HDP).
%
% \subsection{Dirichlet Process}
% Let $A$ be a sample space,  $H$ a base distribution on $A$ and $\alpha$ a positive real number.
% $G$ is a sample from the DP on $A$~\cite{antoniak1974mixtures,ferguson1973bayesian}, i.e. $G \sim \DP(\alpha, H)$, if, for all finite measurable partitions $A_1, \dots, A_k$ of $A$,
% $(G(A_1), \dots, G(A_k)) \sim \Dir(\alpha H(A_1), \dots, \alpha H(A_k))$ holds.
% Even if $H$ is continuous, the drawn distribution $G$ is almost surely discrete. It may be shown that:
% \begin{align*}
% G = \sum_{k=1}^{\infty} \beta_k \delta_{\theta_k} \qquad \{\theta_k\}_{k=1}^\infty   \sim H \qquad \bm{\beta} \sim \Gem(\alpha)\,,
% \end{align*}
% where $\delta_{\theta_k}$ is a Dirac Delta function centred on $\theta_k$.
% Also, $\Gem(\cdot)$, known as a stick-breaking process,
% % \footnote{GEM is named after Griffiths, Engen and McCloskey} can be represented by the \emph{stick breaking process},
% %is analogous to iteratively breaking a portion from the remaining stick which has the initial length $1$. In particular, we write $\bm{\beta} \sim \Gem(\alpha)$ when $u_k \sim \B(1, \alpha)$, $\beta_1 = u_1$, and $\beta_k = u_k \prod_{i=1}^{k-1} (1-u_n)$.
% is analogous to iteratively breaking a portion from the remaining stick which has the initial length $1$. In particular, we write $\bm{\beta} \sim \Gem(\alpha)$ when $u_k \sim \B(1, \alpha)$, $\beta_1 = u_1$, and $\beta_k = u_k \prod_{l=1}^{k-1} (1-u_l)$.
% Theoretically, this is an infinite process as the remaining stick can be arbitrarily small but non-zero.
%
%
% \paragraph{CRP}
% The Chinese Restaurant Process (CRP) is an intuitive and convenient representation of the DP, which we use widely in this work.
% In the CRP, we imagine a Chinese restaurant consisting of an infinite number of tables, each with sufficient capacity to seat an infinite number of customers.
% A customer enters the restaurant and picks one table  at which to sit.
% The $n^{th}$ customer picks a table based on the previous customers' choices.
% That is, assuming  $c_n$ is the table assignment label for customer $n$ and $N_k$ is the number of customers at table $k$, one obtains
% \begin{align}
% p(c_{n+1} = k \mid \bm{c}_{1:n}) =
% \begin{cases}
%   \frac {N_k} {n + \alpha} & \mbox{existing }k \\
%   \frac {\alpha} {n + \alpha} & \mbox{new }k
% \end{cases}
% \qquad
% \theta_{n+1} \mid \bm{\theta}_{1:n} &\sim \frac {\alpha} {n+\alpha} H + \sum_{i=1}^{K} \frac {n_k} {n+\alpha} \delta_{\theta^*_{c_n} } \label{eq:crp-weights} \,
% % \begin{align}
% % \theta^*_{n+1} \mid \bm{\theta^*}_{1:n} &\sim \frac {\alpha} {n+\alpha} H + \sum_{k=1}^{K} \frac {N_k} {n+\alpha} \delta_{\theta_k } \label{eq:crp-weights} \,,
% \end{align}
% where $\bm{c}_{1:n} = \{ c_1, \dots, c_{n} \}$, likewise for $\bm{\theta^*}_{1:n}$.
% The right hand side of~\Cref{eq:crp-weights} indicates how the parameter $\theta^*_{n+1}$ is drawn given the previous parameters, where each $\theta_k$ is sampled from $H$, and $\theta_1, \dots,\theta_K$ are the unique values among $\theta^*_1,\dots,\theta^*_{n}$.
%
%
% \paragraph{Nested CRP}
% To specify the hierarchical mixture model in the manner proposed in the above section we finally need some means of \emph{navigating} through the hierarchy to an appropriate node from which to choose the mixing proportions. For this, we use the \emph{nested} CRP (nCRP)~\cite{blei2010nested}.  In the nCRP, customers arrive at a restaurant and choose a table according to the CRP, but at each chosen table, there is a card leading to another restaurant, which the customer visits the next day, again using the CRP.
% Each restaurant is associated with only a single card. After $L$ days, the customer has visited $L$ restaurants, by choosing a particular path in an infinitely branching hierarchy of restaurants.
%
% \subsection{Hierarchical Dirichlet Process}
% \label{sec:hdp}
% When the number of mixture components is infinite, we connect components along a path in the hierarchy using a HDP.
% The 1-level HDP~\cite{sudderth2006graphical,Teh2006hier} connects a set of DPs, $G_j$, to a common base DP, $G_0$.
% It can be simply written as
% \begin{align*}
% G_j \sim \DP(\gamma, G_0) \qquad G_0 \sim \DP(\gamma_0, H)\,.
% \end{align*}
% It has several equivalent representations while we will focus on:
% \begin{align*}
%   \bm{\beta} \mid \gamma_0 \sim \Gem(\gamma_0) \quad \bm{\beta}_j \mid \gamma, \bm{\beta} \sim \DP(\gamma, \bm{\beta}) \quad \theta_k \mid H \sim H \,,
% \end{align*}
% to obtain $G_0 = \sum_{k=1}^\infty \beta_k \delta_{\theta_k}$ and then $G_j = \sum_k \beta_{jk} \delta_{\theta_{k}}$. Hence $G_j$ has the same components as $G_0$ but with different mixing proportions.
% It may be shown that $\bm{\beta}_j$ can be sampled by firstly drawing $u_{jk} \sim \B(\gamma \beta_k, \gamma(1 - \sum_{\ell=1}^k \beta_\ell))$ and then $\beta_{jk}  = u_{jk} \prod_{\ell=1}^{k-1} (1 - u_{j\ell})$.
%
% Clearly, this process can be extended to multiple levels, by defining another level of DPs with $G_j$ as a base distribution and so on to higher levels. In fact, we can build a hierarchy where, for any length $L$ path in the hierarchy, the nodes in the path correspond to an $L$-level HDP. In such a path, all nodes share the same components as the base DP at the root of the hierarchy but with different mixing proportions, which, for a suitable choice of concentration parameter $\gamma$, tend to become concentrated among fewer and fewer components, the deeper we descend along the path.
% We focus on a HDP along any path rather than a nested DP~\cite{rodriguez2008nested}, since HDPs guarantee that all the descendants and the ancestors share the same components with different weights while nested DPs generate children either identical to each other or totally different regarding both weights and components.
% .



\section{Preliminary}
\paragraph{Dirichlet Process}
We briefly describe the CRP and the stick-breaking process which are two forms of the Dirichlet Process (DP).
% \footnote{
% We brief some technical background in this section.
% For more details, please check out the referenced papers.}

In the CRP, we imagine a Chinese restaurant consisting of an infinite number of tables, each with sufficient capacity to seat an infinite number of customers.
A customer enters the restaurant and picks one table  at which to sit.
The $n^{th}$ customer picks a table based on the previous customers' choices.
That is, assuming  $c_n$ is the table assignment label for customer $n$ and $N_k$ is the number of customers at table $k$, one obtains
\begin{align*}
p(c_{n+1} = k \mid \bm{c}_{1:n}) =
\begin{cases}
  \frac {N_k} {n + \alpha} & \mbox{existing }k \\
  \frac {\alpha} {n + \alpha} & \mbox{new }k
\end{cases}
~~
\theta^*_{n+1} \mid \bm{\theta^*}_{1:n} &\sim \frac {\alpha} {n+\alpha} H + \sum_{k=1}^{K} \frac {N_k} {n+\alpha} \delta_{\theta_k }
\end{align*}
where $\bm{c}_{1:n} = \{ c_1, \ldots, c_{n} \}$, likewise for $\bm{\theta^*}_{1:n}$.
The right hand side indicates how the parameter $\theta^*_{n+1}$ is drawn given the previous parameters, where each $\theta_k$ is sampled from a base measure $H$, and $\theta_1, \ldots,\theta_K$ are the unique values among $\theta^*_1,\ldots,\theta^*_{n}$.


Denoting a distribution by $G$, the stick-breaking process can depicted by
$G = \sum_{k=1}^{\infty} \beta_k \delta_{\theta_k}$, $ \{\theta_k\}_{k=1}^\infty \sim H$ and $\bm{\beta} \sim \Gem(\alpha)$.
Also, $\Gem$ (named after Griffiths, Engen and McCloskey) known as a stick-breaking process,
is analogous to iteratively breaking a portion from the remaining stick which has the initial length $1$. In particular, we write $\bm{\beta} \sim \Gem(\alpha)$ when $u_k \sim \B(1, \alpha)$, $\beta_1 = u_1$, and $\beta_k = u_k \prod_{l=1}^{k-1} (1-u_l)$.


\paragraph{Nested CRP}
In the nCRP~\cite{blei2010nested}, customers arrive at a restaurant and choose a table according to the CRP, but at each chosen table, there is a card leading to another restaurant, which the customer visits the next day, again using the CRP.
Each restaurant is associated with only a single card. After $L$ days, the customer has visited $L$ restaurants, by choosing a particular path in an infinitely branching hierarchy of restaurants.

\paragraph{Hierarchical Dirichlet Process Mixture Model}
\label{sec:hdp}
When the number of mixture components is infinite, we connect components along a path in the hierarchy using a HDP.
The 1-level HDP~\cite{Teh2006hier} connects a set of DPs, $G_j$, to a common base DP, $G_0$.
It can be simply written as
$G_j \sim \DP(\gamma, G_0)$ and $G_0 \sim \DP(\gamma_0, H)$.
It has several equivalent representations while we will focus on the following form:
$\bm{\beta}_0 \sim \Gem(\gamma_0)$, $\bm{\beta}_j \sim \DP(\gamma, \bm{\beta}_0)$, and $\theta_k \sim H$
to obtain $G_0 = \sum_{k=1}^\infty \beta_{0 k} \delta_{\theta_k}$ and then $G_j = \sum_k \beta_{jk} \delta_{\theta_{k}}$. Hence $G_j$ has the same components as $G_0$ but with different mixing proportions.
It may be shown that $\bm{\beta}_j$ can be sampled by firstly drawing $u_{jk} \sim \B(\gamma \beta_k, \gamma(1 - \sum_{\ell=1}^k \beta_\ell))$ and then $\beta_{jk} = u_{jk} \prod_{\ell=1}^{k-1} (1 - u_{j\ell})$.
Considering each data in $x$ belongs to one of the mixture models and in particular $\bm{x}_n$ belongs to the group associated with $G_j$, the 1-level HDPMM is completed by having
$\bm{x}_n \sim F(\theta_{c_n})$ where $c_n \sim \Cat(\bm{\beta}_j)$.
This process can be extended to multiple levels, by defining another level of DPs with $G_j$ as a base distribution and so on to higher levels.
In fact, we can build a hierarchy where, for any length $L$ path in the hierarchy, the nodes in the path correspond to an $L$-level HDP.
% In such a path, all nodes share the same components as the base DP at the root of the hierarchy but with different mixing proportions, which, for a suitable choice of concentration parameter $\gamma$, tend to become concentrated among fewer and fewer components, the deeper we descend along the path.


==> source code/relatedwork.tex <==
\section{Related Work}
We focus on Bayesian methods for the HC.
\cite{stolcke1993hidden} first applied marginal likelihood as the standard for merging the clusters with Agglomerative clustering (AC).
A Bayesian AC with the objective of maximising the \emph{posteriori} was investigated in~\cite{iwayama1995hierarchical}; however, the model assumptions of independence between the data and the clusters are strong.
% \cite{ramoni2002cluster} handled  time series data by maximising the marginal likelihood in an online fashion.
Furthermore, \cite{segal2002prob} presented a Bayesian algorithm assuming that each node associates with a model and similar models should be placed together.
% In another domain,~\cite{friedman2003pcluster} was proposed to doubly cluster the rows and columns in gene data and assign the data entries into a hierarchy.
A Bayesian hierarchical clustering (BHC) that integrates the statistical hypothesis into the traditional AC was proposed in ~\cite{heller2005bhc} and, more
recently, BHC has been relaxed into a non-probabilistic formulation via conjugate-exponential
models~\cite{lee2015bayesian}.
% Interestingly, to address the users' need, an alternative tool is to merge the user interactions into the BHC~\cite{vikram2016interactive}.
However, BHC only provides a Bayesian method of clustering the items into a hierarchy rather than a Bayesian model with a generative process for the data.

In light of hierarchical generative models, an early Bayesian solution introduced the Gaussian tree generative process~\cite{williams2000mcmc}, such that each non-root node is sampled from a Gaussian distribution with the mean of the parent node and predefined level-wise covariances.
The leaf nodes are the observations.
The number of nodes at a certain level is based on a Poisson distribution considering the number of nodes in the parent level.

{\color{red}
A number of works have proposed different but related ways to construct hierarchical tree priors. For example, \cite{Knowles2015} developed the Pitman-Yor Diffusion Tree (PYDT) which is a generalisation of the Dirichlet diffusion tree (DDT)~\cite{neal2003density}.
It assumes that all the observations go through a random walk process from time $0$ to $1$, and each observation has a probability of diverging from the path at the end of each interval of length $dt$ where $0 < dt < 1$.
Finally at time $1$, the data items are sampled from a Gaussian distribution.
With the divergence at different time points, a tree prior is then constructed such that earlier diverging points are the parent nodes of  later diverging points.
In PYDT, the diverging point is also distributed to a Gaussian with the mean of the previous diverging point of the path and some time-related variance.
\cite{teh2008bayesian} proposed applying the Kingman's coalescent as a prior to the HC.
It is in spirit similar to DDT and PYDT, however it is a backward generative process.

A very general way to construct a hierarchical tree prior is proposed in~\cite{adams2010tree} which proposes the tree-structured stick-breaking construction (TSSB) of a hierarchical tree of parameters,  a generalisation of the nested Chinese Restaurant Process (nCRP)~\cite{blei2010nested}.  The method we propose falls within the framework of the TSSB and we discuss in more detail in the next section.}

%They interleave two stick-breaking processes to generate a HC which may maintain observations at internal nodes. It is a very similar configuration to the PYDT, for obtaining parameters for one node from its parent node, although it assumes fixed variance through the path.
%Moreover, the nCRP is largely overlapped by the PYDT and the data can be sampled from internal nodes in the PYDT as well.

\cite{paisley2015nested} discussed the nested Hierarchical Dirichlet Process (nHDP) for topic modelling which, similar to the method we present here, uses the nCRP to navigate through the hierarchy, but associates nodes in the tree with topics. The nHDP first generates a global topic tree using the nCRP~\cite{blei2010nested} where each node relates to one atom (topic) drawn from the base distribution.
\cite{Ahmed2013} also proposed a model that is very similar to nHDP, but appealed to a different inference procedures.
% and applied it in a different scope of applications.

\subsection{Comparison to our Work}
TSSB focuses on Gaussian for the internal nodes in the tree; however, our internal nodes are mixture distributions.
A mixture distribution can handle the data better in many cases, as a single distribution like Gaussian can be considered as a mixture with a single component, and thus the mixture distribution provides more flexibility.
Our implemented model is most closely connected to the TSSB.
Despite its additional complexity, our model still achieves an elegant closed-form updates for the parameters while TSSB needs to apply Hamiltonian Monte Carlo to update the internal parameters in addition to their core slice sampler.

The proposed model exploits the nCRP and HDP and so, at first glance, can appear similar to the nHDP.  It is important to point out that the original nCRP and nHDP are models for hierarchical topic modelling.
Hierarchical topic modelling is well distinguished from HC in~\cite{blei2010nested}.
In HC, the internal nodes are summarisations of the children, while in a topic hierarchy, an internal node reflects the shared terminology of documents associated with the path to that node.  Most notably, a \emph{one-level} HDP is applied in nHDP for projecting a global topic tree to a local, document-specific, one. In contrast, we develop a hierarchy of mixture components and connect these components through a \emph{multilevel} HDP along each path in the hierarchy, thus employing the HDP for a very different purpose.

